Capacity and performance analysis for multi-user system under distributed opportunistic scheduling in a time dependent channel

Consider the problem of a multi-user multiple access channel. While several multi-user coding techniques exist, in practical scenarios, not all users can be scheduled simultaneously. Thus, a key problem is which users to schedule in a given time slot. Under realistic approach for time dependency of the channel, we adopt a distributed scheduling algorithm in which each user, in the beginning of each slot, estimates his channel gain and compares it to a threshold, and if exceeding it the user can transmit. In this work we are interested in the expected capacity of the system and the delay and quality of service of the data accumulated at the users under this scheduling scheme. First we derive the expected capacity under scheduling (distributed and centralized) for this time dependent environment and show that its scaling law is $O(\sigma_g\sqrt{2\log K}+\mu_g)$, were $\sigma_g, \mu_g$ are the good channel parameters (assuming Gaussian capacity approximation, e.g., under MIMO) and $K$ is the number of users. Then we turn to the performance analysis of such system while assuming the users are not necessarily fully backlogged, and focus specifically on the queueing problem and the strong dependence between the queues which leave no alternative but to turn to approximate models for this system. We adopt the celebrated model of Ephremides and Zhu to give new results on the convergence of the probability of collision to its average value (as the number of users grows), and hence for the ensuing system performance metrics, such as throughput and delay. We further utilize this finding to suggest a much simpler approximate model, which accurately describes the system behavior when the number of queues is large. The system performance as predicted by the approximate models shows excellent agreement with simulation results.

==> ModelDescription.tex <==
\chapter{Model Description}\label{model description}

    We consider a slotted MIMO uplink system with $K$ independent users and one base station. The time axis is divided into fixed-length intervals referred to as time slots or, simply, slots, in the sequel. The distribution channel a single user experience, is time varying, as in \cite{gilbert1960}. We assume that a single user, with the strongest received signal at the base station, is selected by a schedular to utilized the channel and transmit in each slot. We are interested in the expected capacity of the system and the delay and quality of service of the data accumulated at the users under this scheduling scheme.\\

    First we analyze the expected channel capacity where the base station chooses the strongest user for transmission using the CSI sent to it from the users. Of course this centralized scheme results in overhead due to the frequently transmissions of the channel state of the users. Then we turn for the capacity analyzing under distributed opportunistic user selection algorithm, which select the strongest user to transmit, without coordinating between the users and without all users sending CSI to the base station. In the distributed scheme we assume that the exact values of the channel matrix $H$ are not available to the transmitter. Yet, the transmitter can approximate it's channel capacity by estimating the SNR of a pilot signal sent from the receiver.\\

    In addition to the system model specification for the capacity part we also specify some assumptions and properties for the QoS part of this study in this section and later in the QoS chapter.\\

    The linear model of the system is:
    \begin{equation}\label{equ-SystemLinearModel}
      \textit{\textbf{y}(n)=H(n)\textbf{x}(n)+\textbf{N}(n)}
    \end{equation}
    $ \textit{\textbf{y}} \in \mathbb{C}^{r} $ is the received vector from the input vector $\textit{\textbf{x}}\in\mathbb{C}^r$ where \textit{H} is a $r\times t$ complex matrix (r - number of receiving antennas, t - number of transmitting antennas) and \textit{\textbf{N}} is zero mean \textit{i.i.d.} complex Gaussian noise with independent, equal variance real and imaginary parts. The transmitter is constrained in its total power to $P$,
    \begin{equation*}
      E[\textit{\textbf{x}}^\dagger\textit{\textbf{x}}]\leq P.
    \end{equation*}

    The matrix $\textit{H}(n)$ is a random matrix which models the Rayleigh fading environment of the time dependent channel.\\

    \section{Time dependent channel}

    The channel distribution each user sees can be modeled as a Markov chain with two states, G (for Good) and B (for bad),where each state determines the channel distribution as can be seen in Figure \ref{fig-GoodBadchannel}.

    \begin{figure}[h]
        \centering
        \includegraphics[width=2in]{gfx/jpeg/BadGoodChannel}
        \caption[Markovian channel model]{Good Bad channel - Markov chain model }
        \label{fig-GoodBadchannel}
    \end{figure}

    We assume that in each slot, each user exist in a good or bad state which is expressed in different channel fluctuations, expressed by Gaussian distribution parameters, respective to the users' state. Given the users' state in each slot, the channel is memoryless conditioned on the state process, hence in each slot the channel capacity is a Gaussian r.v. The dependency of the channel then can be expressed by the dependency between the channel capacity in each slot (\cite{viswanathan1999capacity},\cite{wang1995finite}).
    The capacity of the $i$-th user in each slot, is determined by the Good Bad Markov process $\{J(n)\}$:
    \begin{equation}\label{equ-UserCapacityProcess}
    C_i(n)=
            \begin{cases}
                N_g    & \text{when  } J_i(n)=Good \\
                N_b    & \text{when  } J_i(n)=Bad
            \end{cases}
    \end{equation}
    where $N_g$ and $N_b$ are a random variables distributed normally with parameters $(\mu_g,\sigma_g)$ and $(\mu_b,\sigma_b)$ respectively. This is due to the Gaussian approximation for the MIMO channel capacity as given in Chapter \ref{preliminaries-capacity of MIMO-Gaussian Approximation}. The parameters reflect the differences in the channel qualities, In a way that a good channel parameters maintain $(1) \ \sigma_g>\sigma_b, \ \mu_g,\mu_b\in\mathds{R}$ or $(2) \ \sigma_g=\sigma_b$ and $\mu_g>\mu_b$.\\

    The arrival process of new packages to the system is characterized by a random process, since in this work all user are homogenous we will assume that all user has the same arrival rate $\lambda$. Specifically in the capacity analysis we assume that the users are backlogged, where in the queuing part we assume that new packages may enter the system at any given (continuous) point on the time axis.\\
    The size of the packages is set such that the transmission time is exactly one slot. We define the service time as the time which a package becomes first in the queue until it is successfully transmitted, hence, the service process of the packages composed from the waiting time for transmission and the transmission time. In addition we assume that services are synchronized to (i.e., can only start and end at) slot boundaries, which may cause collisions.










